Selected aspects of complex, hypercomplex and fuzzy neural networks

This short report reviews the current state of the research and methodology on theoretical and practical aspects of Artificial Neural Networks (ANN). It was prepared to gather state-of-the-art knowledge needed to construct complex, hypercomplex and fuzzy neural networks. The report reflects the individual interests of the authors and, by now means, cannot be treated as a comprehensive review of the ANN discipline. Considering the fast development of this field, it is currently impossible to do a detailed review of a considerable number of pages. The report is an outcome of the Project 'The Strategic Research Partnership for the mathematical aspects of complex, hypercomplex and fuzzy neural networks' meeting at the University of Warmia and Mazury in Olsztyn, Poland, organized in September 2022.

==> Artem.tex <==
\chapter{Implementation of neural networks - what has been done and what can be done?}

\addtocontents{toc}{\textit{R.A. Kycia, P. Artiemjew}\par}
\textit{R.A. Kycia, P. Artiemjew}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%Introduction
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\section{Introduction}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
The unprecedented abundance of Artificial Neural Networks (ANN) applications observed in today's world has two main factors. The first one is the growth of computing power related to more advanced hardware progress, including tensor units. The second reason is software dependent - the appearance of easy-to-use, high-level libraries that allows quick to implement various architectures of ANN. These two factors make it easy to construct even very advanced structures and transform the discipline from research to engineering.

There are many architectures of ANN, depending on connection structure. The summary of various approaches is presented in the previous Chapter \ref{Chapter_1}.

In real-life applications, the most common architecture is feed-forward ANN, which consists of layers whose output preceding one serves as input to another layer. Each layer has its specific properties.

For implementation, we focus mainly on Python since it is a leading language used in Machine Learning and applications.

The simplest 'layer' is a perceptron of McCulloch and Pitts \cite{Perceptron_A}. It realizes the division of space of data using a hyperplane (top minus one dimensional) into two disjoint classes - corresponding to both sides of the hyperplane. Therefore, the data that are only hyperplane-separable can be distinguished. The truth table for the XOR logic gate is not hyperplane(linearly)-separable, and this was an input for the first AI winter. The perceptron algorithm is easily implementable from scratch, and it was given in many sources, e.g., Chapter 2 of \cite{Raschka_A}. It is also an easy-to-use implementation as a model \texttt{Perceptron} in Scikit-learn library \cite{PerceptronScikit}.

%There are some noncanonical implementations for other not feed-forward ANN, like Hopfield networks.

Currently, there is also an abundance of sources where there is a description of constructing ANN from scratch \cite{NNFromScratch}. However, to optimize computation, a more advanced approach that uses dedicated libraries is usually needed.


\section{TensorFlow and PyTorch}

The core of today's applications of ANN uses two Open Source libraries\footnote{One library, that, in a sense, was a predecessor and origin of modern libraries was Theano developed at Montreal University\cite{Theano, TheanoPaper}. Currently, it is not popular outside of research applications.}:
\begin{itemize}
\item {TensorFlow \cite{TensorFlow} - released by Google. The current version $2.0$ appeared in 2019. This library is used with high-level API (Application Programming Interface) provided by Keras \cite{Keras}.}
\item {PyTorch \cite{PyTorch} - released by Meta.}
\end{itemize}

Both of them have similar capabilities and philosophies of work, although the architectures of these frameworks are slightly different, mainly because of different algorithms used in various functionalities. Both are based on multidimensional arrays, called tensors\footnote{From the mathematical viewpoint, tensors are algebraic multilinear objects with specific laws of transformation between different bases. This means that they are abstract entities independent of the choice of coordinate frame. Under the particular choice of the frame, they have a form of multidimensional arrays. The notion of a tensor is usually equivalent to the multidimensional array in computer science, and no specific law of transformation is implied.}. Tensors of these two libraries can use CPU, and GPU computing capabilities, including cooperation with CUDA \cite{CUDA} that highly increase the speed of computations. Tensors are structures that can efficiently carry layers of ANN, and each layer is a table of weights for neurons.

Moreover, as discussed in the previous Chapters, the backpropagation algorithm both have automatic differentiation modules (GradientTape for TensorFlow, and AutoGrad for PyTorch).

These libraries also contain various optimizers for backpropagation, as well as numerous additional features allowing preprocessing, postprocessing, and constructing the whole ANN architecture.

The literature about the practical use of both libraries is vast. Therefore we focus on two introductory level books \cite{Raschka_A} for TensorFlow, and \cite{RaschkaPyTorch} for PyTorch.

Both libraries allow to define of custom architectures that employ framework functionality, e.g., automatic differentiation or GPU capabilities.

\section{Non-standard architectures}
We will focus on two examples, from the variety of possibilities, that employ the above libraries to implement non-standard ANN.

The first one uses the PyTorch library to implement the Hopfield layer for the feed-froward network, see \cite{HopfieldPaper_A, HopfieldGithub_A}. It seems that the Hopfield layer is quite universal and incorporates a memory layer that enhances the attention mechanism.

The second implementation we chose is an architecture based on four-dimensional hypercomplex algebra provided in \cite{Marcos} using TensorFlow \cite{MarcosGithub}. The colors are effectively encoded using various four-dimensional hypercomplex numbers. The approach shows exceptionally high accuracy in image classification.


%%%%%%%%%%%%%%%%%%
\section{Conclusions}
%%%%%%%%%%%%%%%%%%
Artificial Neural Networks are fast-developing research and engineering areas. The current implementation standards revolve around two main libraries: TensorFlow with Keras, and PyTorch. Many others, including research, architectures are usually extensions of these two frameworks.

It is very difficult to predict the direction of development of this discipline, including new architectures. However, there is still missing general principle of selecting given architecture of ANN best suitable to analysing specific data under consideration. This is the ultimate goal of this discipline. However, some deeper understanding of ANN at mathematical level is needed first.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\section*{Acknowledgments}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
The article has been supported by the Polish National Agency for Academic Exchange Strategic Partnership Programme under Grant No. BPI/PST/2021/1/00031.

%\appendix




%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%\newpage
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{thebibliography}{00}
\bibitem{Perceptron_A}
W.S. McCulloch, W. Pitts, \emph{A logical calculus of the ideas immanent in nervous activity}, The Bulletin of Mathematical Biophysics, 5(4):115--133, (1943)

\bibitem{PerceptronScikit}
sklearn.linear\_model.Perceptron: \url{https://scikit-learn.org/stable/modules/generated/sklearn.linear_model.Perceptron.html}, Accessed: 16.12.2022

\bibitem{TensorFlow}
TensorFlow, \url{https://www.tensorflow.org/}, Accessed: 16.12.2022

\bibitem{Keras}
Keras, \url{https://keras.io/}, Accessed: 16.12.2022

\bibitem{PyTorch}
PyTorch, \emph{https://pytorch.org/}, Accessed: 16.12.2022

\bibitem{CUDA}
CUDA, \url{https://developer.nvidia.com/cuda-toolkit}, Accessed: 16.12.2022

\bibitem{Theano}
Theano, \emph{https://theano-pymc.readthedocs.io}

\bibitem{TheanoPaper}
Theano Development Team, \emph{Theano: A {Python} framework for fast computation of mathematical expressions}, arXiv: \url{http://arxiv.org/abs/1605.02688}

\bibitem{NNFromScratch}
S. Weidman, \emph{Deep Learning from Scratch: Building with Python from First Principles}, O'Reilly Media, 2019

\bibitem{HopfieldPaper_A}
H. Ramsauer, B. Sch\"{a}fl, J. Lehner, P. Seidl, M. Widrich, T. Adler, L. Gruber, M. Holzleitner, M. Pavlovi\'{c}, G.K. Sandve, V. Greiff, D. Kreil, M. Kopp, G. Klambauer, J. Brandstetter, S. Hochreiter, \emph{Hopfield Networks is All You Need}, \url{https://arxiv.org/abs/2008.02217}

\bibitem{HopfieldGithub_A}
GitHub Hopfield network implementation, \url{https://github.com/ml-jku/hopfield-layers}, Accessed:16.12.2022

\bibitem{Marcos}
G. Vieira, M.E. Valle, \emph{Acute Lymphoblastic Leukemia Detection Using Hypercomplex-Valued Convolutional Neural Networks}, arXiv:\emph{https://arxiv.org/abs/2205.13273} (2022)

\bibitem{MarcosGithub}
Hypercomplex-Valued Convolutional Neural Networks, \url{https://github.com/mevalle/Hypercomplex-valued-Convolutional-Neural-Networks}, Accessed: 16.12.2022

\bibitem{Raschka_A}
S. Raschka, V. Mirjalili, \emph{Python Machine Learning}, Packt Publishing, 3rd edition,  2019

\bibitem{RaschkaPyTorch}
S. Raschka, V. Mirjalili, V. Mirjalili,  \emph{Machine Learning with PyTorch and Scikit-Learn}, Packt Publishing; 1st edition, 2022

\end{thebibliography}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%End
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%



